VeriLA: A Human-Centered Evaluation Framework for Interpretable Verification of LLM Agent Failures

AI practitioners increasingly use large language model (LLM) agents in compound AI systems to solve complex reasoning tasks, these agent executions often fail to meet human standards, leading to errors that compromise the system's overall performance. Addressing these failures through human intervention is challenging due to the agents' opaque reasoning processes, misalignment with human expectations, the complexity of agent dependencies, and the high cost of manual inspection. This paper thus introduces a human-centered evaluation framework for Verifying LLM Agent failures (VeriLA), which systematically assesses agent failures to reduce human effort and make these agent failures interpretable to humans. The framework first defines clear expectations of each agent by curating human-designed agent criteria. Then, it develops a human-aligned agent verifier module, trained with human gold standards, to assess each agent's execution output. This approach enables granular evaluation of each agent's performance by revealing failures from a human standard, offering clear guidelines for revision, and reducing human cognitive load. Our case study results show that VeriLA is both interpretable and efficient in helping practitioners interact more effectively with the system. By upholding accountability in human-agent collaboration, VeriLA paves the way for more trustworthy and human-aligned compound AI systems.

==> tex/00_abstract.tex <==
% \begin{abstract}
% This paper introduces the design and evaluation of large language model (LLM)-based AI agents for human-agent interaction, focusing on assisting AI practitioners in assigning task decomposition to AI agents. Our proposed framework, \name{} (\textbf{Veri}fiable \textbf{T}ask \textbf{D}ecomposition), enables LLM agents to autonomously self-verify erroneous execution results during task decomposition. We first define clear task expectations and apply the evaluation module based on human standards. By leveraging the evaluation module for each agent, we assess the granularity of each agent's performance and its impact on the final agent's result. To ensure that execution quality aligns with human standards, we integrate human-driven criteria that evaluate features such as accuracy, format adherence, and contextual sufficiency in our evaluation module. 
% This approach enhances the interpretability of agent-based systems for humans, clarifying why an agent may have failed, providing clear guidelines for revision, and reducing the user's cognitive load. Thus, agents can better align with user expectations in systems requiring task propagation. Our framework paves the way for future agent-driven systems that meet users' needs, encouraging greater accountability in agent-human collaboration.
% \end{abstract}
